The Metaverse: Survey, Trends, Novel Pipeline Ecosystem & Future Directions

The Metaverse offers a second world beyond reality, where boundaries are non-existent, and possibilities are endless through engagement and immersive experiences using the virtual reality (VR) technology. Many disciplines can benefit from the advancement of the Metaverse when accurately developed, including the fields of technology, gaming, education, art, and culture. Nevertheless, developing the Metaverse environment to its full potential is an ambiguous task that needs proper guidance and directions. Existing surveys on the Metaverse focus only on a specific aspect and discipline of the Metaverse and lack a holistic view of the entire process. To this end, a more holistic, multi-disciplinary, in-depth, and academic and industry-oriented review is required to provide a thorough study of the Metaverse development pipeline. To address these issues, we present in this survey a novel multi-layered pipeline ecosystem composed of (1) the Metaverse computing, networking, communications and hardware infrastructure, (2) environment digitization, and (3) user interactions. For every layer, we discuss the components that detail the steps of its development. Also, for each of these components, we examine the impact of a set of enabling technologies and empowering domains (e.g., Artificial Intelligence, Security & Privacy, Blockchain, Business, Ethics, and Social) on its advancement. In addition, we explain the importance of these technologies to support decentralization, interoperability, user experiences, interactions, and monetization. Our presented study highlights the existing challenges for each component, followed by research directions and potential solutions. To the best of our knowledge, this survey is the most comprehensive and allows users, scholars, and entrepreneurs to get an in-depth understanding of the Metaverse ecosystem to find their opportunities and potentials for contribution.

==> src/ResearchDirections.tex <==
Following the list of challenges described above, we conclude that the current development for building and deploying the Metaverse is still in the first stages. As a step towards addressing some of these challenges, we present, in this section, a detailed study of potential impactful and effective research directions. Our presented directions are a result of a thorough study of the current demands to empower immersiveness and realism in the Metaverse ecosystem. 
In this section, we present the list of directions targeting each component in our proposed multi-layer pipeline architecture of the Metaverse development. In Figure \ref{fig:metaverse_directions}, we summarize these directions.

\begin{figure}
    \centering
    \includegraphics[scale=0.21]{images/metaverse_directions.drawio.png}
    \caption{Future directions per component in the Metaverse ecosystem}
    \label{fig:metaverse_directions}
\end{figure}

\subsection{Hardware \& Equipment}
Existing Hardware and Equipment for supporting the creation, development, and deployment of the Metaverse are still in their infancy. Research is required to develop new display technologies, such as holographic and light-field displays, to improve realism and immersiveness using VR and AR technologies \cite{chen2019overview}. In addition, research on new technologies for building input devices is required, such as gloves or full-body suits. In addition, accessibility should be addressed by research on new techniques to support people with disabilities to use the Metaverse. This is possible through improving haptic feedback and utilizing eye-tracking technologies. It is also important to support voice recognition and control by improving its accuracy and responsiveness. Moreover, sensors on hardware and equipment require additional improvement to maintain stable accuracy by improving calibration algorithms and utilizing machine learning. Furthermore, the sensors' range and flexibility should be improved, which is important for motion-capturing devices. Range and flexibility can be increased by improving the speed and quality of the signal processing algorithms while incorporating and optimizing the use of additional sensors \cite{chen2019study}. Concerning manufacturing, hardware and equipment production must adhere to sustainability and eco-friendly requirements. Moreover, the energy utilization of devices should be further studied by investigating the use of low-power components, such as processors and displays. It is also possible to reduce the energy usage on the devices by resorting to the cloud or fog for faster computing and developing power management software on these devices. 

\subsection{XR Frameworks}
In order to reflect on the challenges discussed over the XR frameworks, several aspects of potential direction and measures can be taken to lessen them and suggest potential solutions to ensure a positive experience for both developers and end users. An important direction is to adopt standards and protocols, ensuring that various XR frameworks and systems may communicate and interact with one another through developing and creating open-source libraries or APIs. Another direction is to create XR experiences that are simple and intuitive for users to understand by incorporating user feedback into the design and development process. Furthermore, creating new networking protocols and technologies that are more effective and resistant to latency and bandwidth limitations could improve network performance \cite{cheng2022will}. Moreover, the XR framework should offer solutions for the increased complexity of supported applications through dynamic scaling approaches and improving compatibility measures. Besides, real-time movements and tracking synchronization are vital for supporting interoperability, which is possible by developing standards to be adapted across these framework creators. In addition, maintaining the security and privacy of users' data by implementing a security mechanism that limits access to adversaries, such as encryption and authentication procedures, and ensures compliance with security legislation. Finally, creating AI models and algorithms that are transparent and accountable, and take into account diversity and inclusion during the data collection and training processes \cite{cao2022decentralized}. AI-based solutions should be developed to support social interactions by developing advanced natural language models and tools. Therefore, collaboration among specialists from different fields is vital in improving the XR framework development and usage.

\subsection{Platforms \& MaaS}
The back end forming the backbone of Metaverse platforms and services requires flexibility and scalability in terms of computing and networking performance. Therefore, the Quality of Service (QoS) can be improved by integrating the use of cloud and fog computing that utilize containers and micro-services architectures for seamless on-demand deployment \cite{sami2020dynamic, sami2021demand}. Through a distributed on-demand fog and edge computing architecture, the computing and networking load are reduced between Metaverse users and the cloud, relaxing resource utilization. Furthermore, it is important to develop resource management solutions, ensuring effective and efficient dynamic and scalable service placement, host selection, and horizontal and vertical resource scalability \cite{sami2021ai}. Resource management for supporting the Metaverse requires proactive and demand-driven decisions. As a potential direction, Reinforcement Learning (RL) and reward shaping solutions can be developed on top of an environment modeling design to meet the resource management requirement for Metaverse platforms and MaaS. Moreover, networking protocols should be offered and adapted to the platforms and services to ensure packet delivery by developing advanced traffic engineering, network slicing, and quality-based routing mechanisms. Furthermore, reducing latency and improving content delivery through caching mechanisms are of immense importance. Therefore, additional resources must be dedicated to developing Content Delivery Network (CDN) solutions for faster and more reliable delivery, by caching the content closer to users \cite{zolfaghari2020content}. Using CDN, requests are routed to the nearest server in the network that has a copy of the content. On another end, applications on platforms and algorithms running behind the services can be improved by utilizing Quantum Computing. Applications of Quantum Computing as tools to support the Metaverse platforms and MaaS developments include: (1) optimization towards rendering; (2) physics and environment simulation to study and improve the user experience; (3) advancement and security in computing and networking architectures; and (4) Quantum AI can be used to optimize the machine learning solutions and autonomous agents for a more immersive experience. Moreover, providers of the Metaverse platforms and services should manage content creation and offer curation tools to find and share relevant content that is more user-friendly. This is possible by offering solutions for digital assets management, content discovery, social sharing, and collaborative curation. With regards to controlling user behaviors, research can focus on developing gamification solutions that can incentivize virtual users or avatars to promote positive behavior and engage in the environment. Furthermore, new research directions should focus on user identification and building trust in cross-platform environments, where users can interpolate platforms to immersive different experiences \cite{wang2022survey}. This is possible through (1) developing distributed cross-chain solutions, (2) utilizing a reputation mechanism, (3) utilizing multi-factor authentication (MFA), and (4) partnering with trust identity providers, such as government agencies or banks.

\subsection{Avatars}
In the future, it is expected that users might care more about their appearances in the Metaverse vice the real or physical world. The first impressions of users entering the Metaverse are driven by their look and appearance as avatars. Therefore, it is necessary to address the existing challenges related to avatars creation, movement, and management to enable the basic requirements for users as part of their Metaverse experience and onboarding. A research direction concerning avatar creation and modeling is to use machine learning generative models for more customizable and realistic avatars \cite{harshvardhan2020comprehensive}. This includes learning models for creating faces, textures, clothing, and voice tone adjustments. Existing advancements in convolutional and recurrent neural network design are a promising start for building such solutions. Furthermore, 3D scanning of the physical appearance of the user can be used for realistic avatar creation \cite{dixit2019tool}. The first step in 3D scanning for avatar creation is to perform scanning of physical appearance using photogrammetry software or just smartphones. The second step involves modeling, where scanned users are transformed into 3D digital representations subject to customization and adjustments. The last two steps include texturing (skin, hair, and clothes) and animation of the avatars to simulate realistic movements and interactions. Animation can be performed with the support of AI that utilizes motion capture to develop procedural animation systems, lip-syncing with mouth movements, and facial animation and expressions. In terms of animation, using advanced device sensors involves transmitting the sense of touch in addition to visual or audio feedback. The sensation for improving animation requires further integration and support of haptic feedback, tactile, and temperature sensors in the platforms, In addition, using biometric data, avatars become more realistic with automated personalization features \cite{gavrilova2011applying}. For instance, facial features can be accurately represented on the avatar face by using face recognition mechanisms, which result in real-time face animation. Moreover, the user voice can be analyzed for identity verification and the development of self-learning and adaptive AI models to create avatars that speak like the real user while controlling expressions and mouth movements. Furthermore, integrated biometric sensors in input devices can be used to capture physical states or movements. For instance, reading heart rate can be reflected in the avatar state in the Metaverse. 
In terms of security and privacy aspects, it is important for regulation on personal data acquisition to be updated accordingly. Additionally, applications should implement robust security measures to protect personal data, as well as be transparent about how the data is being used \cite{buck2022security}. 
Finally, ethical and social implications must be carefully investigated through a set of rules and regulations to avatar design implications and behaviors in the Metaverse.

\subsection{Rendering}
To address the challenges posed by existing rendering engines in the context of the Metaverse, we present a list of directions that can improve the quality, speed, and performance of rendering solutions. For addressing the need for realistic rendering of light in the Metaverse, the ray tracing rendering technique can be used and augmented for supporting the high complexity in the Metaverse environments. Ray tracing is computationally expensive but results in realistic light simulation by respecting the underlying physics of different materials and surfaces \cite{he2018design}. For addressing the issue of performance and increased delays by rendering engines in the Metaverse, research should focus on advancing existing hardware technology and consider performing distributed rendering. More specifically, multiple computing machines can be used to render a single scene, which helps reduce the amount of time and resources required for rending. Another direction can be developed by relying on AI techniques to support scene rendering in the Metaverse \cite{tewari2020state, jing2019neural}. In this regard, AI can be used to optimize the rendering settings and resources required without sacrificing the quality. Besides, AI and heuristics can be used to cache content for streaming by studying the virtual user behavior and predicting the need for rendering to act proactively and avoid latency. Furthermore, rendering engine performance can be improved by investigating the use of procedural generation in the context of Metaverse, where content is generated on the fly \cite{liu2021deep}. For instance, procedural generation can be used to generate textures and models, which reduces the need for large storage or high computation power. Moreover, photogrammetry can be employed to create 3d models of objects with enhanced quality textures and details.  As a result, effective resource allocation is necessary to maximize service delivery performance to a large number of users at the edge. 

\subsection{Sessions}
In the context of sessions and data management for the complex Metaverse environment handling millions of concurrent users, some technological contributions need to be explored to address existing challenges. The first direction would include investigating a set of distributed data storage mechanisms for managing sessions in highly loaded environments. In this context, data will be stored across distributed servers to improve accessibility and redundancy. Consequently, data retrieval can be improved as a result of parallel queries from distributed storage. In this regard, effective distributed storage and retrieval mechanism should be investigated, where AI mechanisms can be effective. Solutions to achieve distributed storage are to use distributed (1) cloud computing, (2) edge and fog computing, (3) Content Delivery Networks (CDN), and (4) Blockchain-based storage. Cloud computing offers automatic scaling and load balancing of storage and data analysis compared to on-premise servers (i.e., edge and fog servers). Furthermore, edge and fog servers offer reduced network utilization and latency, as well as fast analysis and reduced loads on external servers. 
To this end, a hybrid architecture is most likely to be the effective approach; however, several proposals should be designed per solution to obtain its full potential (i.e., divide and conquer strategy). Additionally, CDN can be used to deliver session-related information to users to reduce latency and computation on the Metaverse infrastructure. Besides, Blockchain is a distributed ledger technology that uses distributed storage by nature and requires a consensus mechanism for approving the addition of data in the form of transaction blocks. Thus, the use of Blockchain for managing sessions would improve distributed storage and retrieval, in addition to adding a robust security layer to protect user data \cite{cao2022decentralized}. The role of AI is major in managing the computing infrastructure of each of these solutions. In this regard, AI can be used for automatically managing resources on-demand by studying the change in loads and acting proactively for assigning storage and distributing analysis tasks while performing intelligent vertical and horizontal scaling and load balancing \cite{sami2021ai}. Furthermore, AI is the primary tool adapted to create personalized experiences by offering user sessions that adapt to user preferences. For instance, reinforcement learning and recurrent neural network can be used to create adaptable models that study the change in preferences over time. Besides, serverless Metaverse services bring additional flexibility and performance improvement due to the ability to create and delete instances on the fly, assign additional storage capacity, and reduce the cost of management \cite{li2022serverless}. Hence, serverless computing and storage architectures are promising and should be properly investigated.\\
To further improve the efficiency and cost of data storage, data compression mechanisms can be employed \cite{jayasankar2021survey}. Data compression, when effective, is guaranteed to reduce latency and improve the performance of data flow management and transmission. On another note, quantum computing combined with AI (i.e., Quantum AI) is promising to reduce and optimize the computation through faster processing of session data.\\
Finally, advanced networking architecture is required to support data management and transmission. Therefore, the 6G network perspective and contributions can be used to examine the resource heterogeneity problem between different devices, while supporting session synchronization and reliability.
% Regarding session data collection and usability, the method by which personal data will be treated should be explicitly specified.

% Furthermore, whether the data will be obtained by a single administrator or through a decentralized system in which many agencies access session data must be decided.

% Furthermore, studies on the impact of data breaches on consumers can be valuable. Session data may be used to manage resources, for example, by generating a session before requesting it.

% The 6G network perspective and contributions can be used to examine the resource heterogeneity problem between different devices, and it impacts session synchronization and reliability. Additionally, the role of AI in session resource optimization and scalability should be examined more. For example, AI could be applied to predict how many people would attend a particular session based on previous historical data. Finally, AI can help determine the number of sessions that will be launched.

\subsection{User-to-User Interactions}
For addressing the existing challenges entailing user-to-user interactions in the Metaverse, there is a need for collaboration among multiple companies and regulators. Furthermore, efforts are required to state the guidelines for such a type of interaction, especially when hosting an environment for multicultural users. Empowering social presence among avatars in the Metaverse is of immense importance for achieving immersiveness and engagement in the virtual space. Social presence can be achieved in different ways. One of them is implementing spatial audio to improve interactions and create a sense of presence \cite{kim2019immersive}. There are several steps to implement spatial audio, which include (1) capturing data, (2) creating a virtual audio environment, (3) assigning audio sources, (4) simulating sound propagation, and (5) rendering the audio stream in the virtual space. In addition, social network analysis and optimization can be achieved using AI technologies for learning and improving past and undergoing users' interactions in the environments, thus leading to an increased quality of experience \cite{laurell2019exploring}. Furthermore, utilizing avatars that mimic emotions and expressions enriches the social presence experience for Metaverse users. Another important research direction is to investigate non-verbal communication techniques, such as text or sign language, for voice propagation accessibility.\\
Tracking and sensing technologies can also improve user-user interactions and immersiveness by achieving accurate and responsive rendering feedback during communications. Investigating advanced tracking and sensing technologies leads to improving body tracking, gesture recognition, eye tracking, and haptic feedback.\\
Another method to improve user-to-user interactions is by creating virtual agents or assistants and utilizing natural language generation (NLG) \cite{gatt2018survey}. In specific, virtual assistants support avatars and guide them to navigate the Metaverse and perform actions. NLG and agents can also be used for real-time translation to overcome the barrier of multi-cultures and communications. NLG can be used to generate natural-sounding speech based on the interaction context, thus empowering more engagement and dynamicity.


\subsection{User-to-Business Interactions}
There exist multiple challenges for this category of interaction affecting businesses and the quality of experience delivered. In this section, we present a list of research directions that can potentially address some of these challenges. Starting with the infrastructure limitations, there is no clear mechanism for identifying the available computing and networking infrastructure and how to use it by each. Henceforth, a clear study about the management and scheduling of such resources is essential, while considering fairness and trust among applications and customers. Furthermore, the Metaverse is hungry for resources, thus providing fair allocation and innovative coordination between the physical and virtual worlds for sharing network and computing resources is necessary. More specifically, computing resources should be allocated fairly to cope with the increase in demands as users start relying more on Metaverse to engage socially and perform daily tasks \cite{sami2021demand}. Moreover, the use of cloud, fog, edge, and CDN resources and technologies would essentially improve the support for businesses in the Metaverse. Through business-to-business collaboration, various challenges can be conquered.\\
From a user perspective, a research direction should consider building and managing the virtual economy of businesses, as well as transactions in the Metaverse \cite{popescu2022augmented}. One step is to motivate the creation of virtual showrooms for shopping, browsing virtual products, and hosting events for brand management. Furthermore, virtual assistants can be created through the help of AI with customized user experience to help create a trusted bond and relationship between customers and businesses \cite{lee2022toward}. Those assistants can also be used as customer support agents for managing users' complaints. Virtual marketing and immersive advertisement strategies are also important for supporting virtual businesses and building a powerful economy. This also entails using the Metaverse for product design and prototyping \cite{escalada2019design}. Powerful rendering engines are also promising for managing the complete supply chain in the Metaverse, which has a positive impact on businesses. For instance, supply chain management in the Metaverse can include tracking inventory and performing required logistics in real-time. Furthermore, the Metaverse can help businesses in expediting training and onboarding sessions for new employees while facilitating team building and enabling remote work opportunities \cite{kral2022virtual}.\\
On another note, the use of Blockchain technology by businesses empowers secure and transparent digital commerce to motivate the actions of buying, selling, and trading virtual goods. Moreover, interoperability raises additional challenges, including ways to teleport required data across various environments, establish reliable connectivity with distant servers, monitor and maintain access, and standards for financial exchange. In this regard, the Blockchain can be used to address some of the interoperability challenges by employing a cross-chain technology with a consortium Blockchain between partners.

\subsection{User-to-Object Interactions}
Promising potential solutions to the existing limitations as a result of user-to-object interactions are many folds. First, developing on-demand fog and edge computing layers next to users leads to rendering real-time personalized experiences, this accounting for DT requirements. Consequently, fewer network and computing resources are consumed by transferring the load to neighboring servers. Furthermore, it is essential to integrate advanced, fast, and scalable AI techniques to decide on the right time and place to deploy the on-demand fog servers and perform the required resource scheduling \cite{sami2021ai}. In addition, AI solutions can advance the rendering capabilities by pre-rendering interactions with objects by studying users' behaviors and predicting the next needed object manipulation inside the Metaverse. Besides resource management and proactive decision-making, AI has great potential in providing assistance for users to facilitate user-to-object interactions. This includes the role of AI to process voice commands and provide personalized interaction experiences. Furthermore, an improvement in sensory technology combined with the power of AI can improve the accuracy of object tracking to reduce latency in manipulation. Furthermore, combined with Blockchain, AI can be used to create a smart distributed ownership management system, adding an additional layer of security and transaction management mechanism \cite{cao2022decentralized}. Additionally, using AI, utilizing swarm robots is another promising solution for elevating the interactions with objects, where robots can collaborate together to process and handle users' commands and feedback. Furthermore, gamification can be utilized with an AI synergy in order to motivate users through rewards to interact more with the surrounding, thus increasing engagement inside the Metaverse.\\
Achieving real-time synchronization of objects and environment manipulation between the real and physical world, in addition to studying the surroundings in the case of augmented reality requires additional research. Potential research directions consist of developing mechanisms for (1) accurate tracking, (2) real-time mapping, and (3) dynamic object placement \cite{park2020augmented}. For advancing tracking accuracy, techniques such as computer vision and sensor fusion can be used. Moreover, real-time mapping can be achieved using advanced sensors that can capture detailed information about the environment, including Li-DAR and depth cameras.\\
Another promising track of research is the use of generative design to enhance user-to-object interaction \cite{keshavarzi2020v, jennings2022generativr}. Using the generative design, the following features are guaranteed: (1) customization, (2) efficiency, (3) realism, and (4) innovation. In particular, generative models empower personalized user experiences by providing a tool for customizing objects in relation to preferences. Besides, efficiency is guaranteed by optimizing the design of the objects in the Metaverse, leading to less resource utilization for rendering and post-interaction manipulation. In addition, generative models enable realistic object design with an increased margin of innovation by providing a wider range of implementing designs. Therefore, generative design is promising and can push the boundaries of efficiency, realism, and innovation.\\
Furthermore, it is essential to integrate the use of Blockchain, which is integrated and shared across Metaverse environments, where users can easily share and transfer objects ownerships (e.g. using the cross-chain concept). Furthermore, a set of regulations and guidelines must be outlined, shared, and adapted by all Metaverse owners or managers to make sure that all objects and features for available interactions and services are available for everyone and not limited to a group of users.\\
Finally, with the increase in diversity and need for additional object designs, it is essential to share a public repository including large libraries of design and manipulation options. Moreover, the Metaverse can be used to provide training for new users joining and teach them about the existing types of interactions and experiences.
